PANAS-t: A Pychometric Scale for Measuring Sentiments on Twitter

Online social networks have become a major communication platform, where people share their thoughts and opinions about any topic real-time. The short text updates people post in these network contain emotions and moods, which when measured collectively can unveil the public mood at population level and have exciting implications for businesses, governments, and societies. Therefore, there is an urgent need for developing solid methods for accurately measuring moods from large-scale social media data. In this paper, we propose PANAS-t, which measures sentiments from short text updates in Twitter based on a well-established psychometric scale, PANAS (Positive and Negative Affect Schedule). We test the efficacy of PANAS-t over 10 real notable events drawn from 1.8 billion tweets and demonstrate that it can efficiently capture the expected sentiments of a wide variety of issues spanning tragedies, technology releases, political debates, and healthcare.

==> detecting.tex <==
\subsubsection{Computing the PANAS-t score}

Tweets expressing certain sentiments can be much more popular than others. Thus,  in order to tell if a sentiment has increased or decreased for a specific event (e.g. Michael Jackson's death) we first need a baseline for comparison. A natural baseline consists of the whole dataset of normalized of tweets. Thus, by quantifying the fraction of tweets that are related to each sentiment using this baseline we will be able to tell if a sentiment increased for a specific event \textit{related} to the presence of this sentiment in the entire dataset. Next, we detailed describe how we compute this baseline for comparison. 

\begin{table}[b]
			\centering
			\small
				\begin{tabular}{ | l | r |}
				\hline
				\textbf{Sentiment ($s$)} & Baseline (\textbf{ $alpha_s$})\\
				\hline
				\hline
				
				Fear & 0.0063791\\
				\hline
				Sadness & 0.0086279\\
				\hline
				Guilt & 0.0021756\\
				\hline
				Hostility & 0.0018225\\
				\hline
				Shyness & 0.0007608\\
				\hline
				Fatigue & 0.0240757\\
				\hline
				Surprise & 0.0084612\\
				\hline
				Joviality & 0.0182421\\
				\hline
				Self-assurance & 0.0036012\\
				\hline
				Attentiveness & 0.0008997\\
				\hline
				Serenity & 0.0022914\\
				
				\hline
				\end{tabular}
				\caption{Fraction of tweets for each sentiment in the entire dataset.}
				\label{tab:table3}
\end{table}

Each tweet in the normalized set of tweets was mapped to a single sentiment.  To do that, when an adjective from Table~\ref{tab:table2} associated with a certain sentiment $s$ appears as one of the terms of a normalized tweet, we considered that tweet associated to sentiment $s$. In cases of tie we associated to the tweet the first sentiment identified in the normalized tweet. However, cases of tie were very rare and are negligible to our quantities. Based on this information, we define the baseline values for each sentiment as
follows.

Let $T$ be the entire set of normalized tweets and $T_s$ the subset of these tweets related to sentiment $s$. Thus, the baseline value for each sentiment, $\alpha_s$, is defined as $\alpha_s = |T_s| / |T|$.  In other words, we simple divide the occurrence of tweets of each sentiments by the total number of normalized tweets in our dataset. Table~\ref{tab:table3} shows the baseline values for the occurrence of each sentiment considered.  We can note that some sentiments occur orders of magnitude than others. For instance, tweets expressing \textit{fatigue} occurs about 32 more times than tweets expressing \textit{shyness}, which reinforces that a normalization is required.

Based on these values, we can compute the relative increase or decrease in sentiments for a particular sample of tweets as follows.  Let $S$ be a set of tweets (e.g. a sample of tweets related to Michael Jackson's death) and $S_s$  the subset of these tweets related to sentiment $s$. We define $\beta_s$ as $\beta_s = |S_s| / |S|$. Then, we define the PANAS-t score as an eleven-dimensional sentiment vector, where the PANAS-t score function $P(s)$ can be computed as bellow:

\[
 P(s) =
  \begin{cases}
   (\alpha_s - \beta_s)/\alpha_s 						&\text{if } \beta_s \le {\alpha_s} \\
   -1(\beta_s - \alpha_s)/\beta_s				  &\text{if } \beta_s \textgreater{\alpha_s}
  \end{cases}
\]

Based on this strategy, each $P(s)$ value can vary from -1 to 1 for each sentiment.  An event with $P(fear)$ = 0 means that the event has no increase or decrease for the sentiment \textit{fear}, in comparison with the entire dataset of tweets posted as of 2009.  A positive value of 0.3 would mean an increase of 30\%, and so on.

Our strategy to compute the PANAS-t score is simple and suitable for allowing the comparison of both, increase and decrease of each sentiment relatively to a non-bias dataset. More important, Table~\ref{tab:table3} provides a baseline for comparison of any kind of sample of tweets.  For instance, one could easily crawl a sample of tweets from the Twitter API
and use those values to normalize the sentiment scores. 

